Fex: Assisted Identification of Domain Features from C Programs

Modern software typically performs more than one functionality. These functionalities or features are not always organized in a way for modules representing these features to be used individually. Many software engineering approaches like programming language constructs, or product line visualization techniques have been proposed to organize projects as modules. Unfortunately, much legacy software suffer from years or decades of improper coding practices that leave the modules in the code almost undetectable. In such scenarios, a desirable requirement is to identify modules representing different features to be extracted. In this paper, we propose a novel approach that combines information retrieval and program analysis approaches to allow domain experts to identify slices of the program that represent modules using natural language search terms. We evaluate our approach by building a proof of concept tool in C, and extract modules from open source projects.

==> background.tex <==
\section{Background}
\label{sec:background}
In this section, we provide some background on
the information retrieval\footnote{We don't go into mathematic details, which are beyond the scope of this paper} and data-flow analysis techniques on which our approach builds.


\subsection{Information Retrieval}
%In this subsection, we will briefly describe the various foundational information retrieval concepts used by our approach without going into the detailed mathematics, which are beyond the scope of this paper. 
Below, we briefly overview IR concepts that we use in the rest of the paper. 



\subsection{Data-flow analysis} 
Reps, Horwitz and Sagiv~\cite{repspopl} introduced the \textbf{IFDS} framework to solve inter-procedural, finite, distributive subset (IFDS) problems. Given the IFDS framework, designers of data-flow program analyses need only define a set of flow functions, which the framework solves. \textbf{Phasar}~\cite{boddenphasar} is an LLVM based static analysis framework for C++ with in-built support for IFDS. In order to define a program analysis using Phasar, we need to implement the following four functions, illustrated in Figure~\ref{fig:flowfunctions}\footnote{\url{https://github.com/secure-software-engineering/phasar/wiki/Writing-an-IFDS-analysis}}:
\begin{enumerate}
\item \textbf{getNormalFlowFunction}: The analysis developer uses this
function to express what happens during intra-procedural data flows. An example of this is indicated by the green arrow between the use of \texttt{a} and the definition of \texttt{a} in Figure~\ref{fig:flowfunctions}.
\item \textbf{getCallFlowFunction}: The analysis developer uses this function to express what happens when a call-site is encountered, i.e., how to handle the relationship between the actual parameters and the formal parameters of a function. In Figure~\ref{fig:flowfunctions}, an example of such kind of flow is between the actual parameter \texttt{b} and the formal parameter \texttt{b\_x} indicated by the black arrow. 
\item \textbf{getRetFlowFunction}: The analysis designer uses this function to indicate how to handle the flow from a return statement to the variable the return value is assigned to. An example of this kind of flow in Figure~\ref{fig:flowfunctions} is the return statement of \texttt{foo} to \texttt{a} indicated by the blue arrow. 
\item \textbf{getCallToRetFlowFunction}: The analysis designer uses this function to indicate how to handle things like pointer parameters, that is not handled by the function call. \todo{last part of the sentence is broken... }
\end{enumerate}

\begin{figure}
\includegraphics[scale=0.35, left]{images/flow.png}
\caption{Flow functions}
\label{fig:flowfunctions}
\end{figure}

\subsection{Single Static Assignment - SSA}
Single static assignment(SSA)~\cite{braunssa} is a popular attribute of any intermediate representation of code, that emphasizes that each variable be assigned only once. The advantage is that optimizations are simplified and analyzing properties of variables are facilitated. Phasar provides an SSA representation of the LLVM IR, which we use to make our analysis more efficient. Consider the following code snippet:
\begin{tcolorbox}
a = 10;\\
a = 20;\\
b = a;
\end{tcolorbox}

Although to the naked eye, it is obvious that first assignment of \texttt{a} is unused, for a static analysis, it would require tracing the definitions of \texttt{a} to arrive at this understanding. 
Now, consider the SSA form of the same code snippet:

\todo{I would put the two versions of code side-by-side ...}
\begin{tcolorbox}
a1 = 10;\\
a2 = 20;\\
b1 = a2;
\end{tcolorbox}

Making such an analysis would be free. 

==> impl.tex <==



